Enhanced Euclidean supersymmetry, 11D supergravity and $SU(\infty)$ Toda equation

We show how to lift solutions of Euclidean Einstein-Maxwell equations with non-zero cosmological constant to solutions of eleven-dimensional supergravity theory with non-zero fluxes. This yields a class of 11D metrics given in terms of solutions to $SU(\infty)$ Toda equation. We give one example of a regular solution and analyse its supersymmetry. We also analyse the integrability conditions of the Killing spinor equations of N=2 minimal gauged supergravity in four Euclidean dimensions. We obtain necessary conditions for the existence of additional Killing spinors, corresponding to enhancement of supersymmetry. If the Weyl tensor is anti-self-dual then the supersymmetric metrics satisfying these conditions are given by separable solutions to the $SU(\infty)$ Toda equation. Otherwise they are ambi-K\"ahler and are conformally equivalent to K\"ahler metrics of Calabi type or to product metrics on two Riemann surfaces.

==> papers_macros_1.tex <==
\newcommand{\NN}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\CP}{\mathbb{CP}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\RP}{\mathbb{RP}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\X}{\mathbb {X}}
\newcommand{\DD}{\mathbb {D}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\bK}{\mathbb{K}}

\newcommand{\Rho}{\mathrm{P}}
\newcommand{\N}{\mathbb{N}}

\def\Ub{{\widetilde U}}
\def\Nb{{\widetilde N}}
\def\ep{{\varepsilon}}
\def\dom{\delta \Om}
\def\tom{\tilde{\omega}}
\def\Ddot{\delta \Theta}
\newcommand{\lam}{\lambda}

\let\a=\alpha 
\let\b=\beta

\def\bfA{{\bf \Omega}}
\def\pr{{\bf pr}}

\def\t{\tilde}
\def\ov{\overline}
\def\co{\mbox{const}}
\def\p{\partial}
\def\k{\kappa}
\def\g{\mathfrak{g}}
\def\pr{{\bf pr}}
\def\opsi{\overline{\psi}}
\def\ophi{\overline{\phi}}
\newcommand{\et}{\tilde{\textbf{e}}}
\def\II{{\cal{I}}}

\def\TH{
\left (
\begin{array}{cc}
\p _y& \p _w+\Th_{yy}\p _x-\Th _{xy}\p_y  \\
-\p_x&\p _z-\Th _{xy}\p _x + \Th _{xx}\p_y
\end{array}
\right ) 
}
\def\OM{
\left (
\begin{array}{cc}
\Om _{w\wt}\p _{\zt}-\Om _{w\zt}\p _{\wt}&\p_w \\
\Om _{z\wt}\p _{\zt}-\Om _{z\zt}\p _{\wt}&\p_z
\end{array}
\right ) 
}

\def\Nb{{\widetilde N}}
\def\Bb{{\widetilde B}}
\def\Ab{{\widetilde A}}
\def\mm{|\mu|}
\def\vol{{d{\bf x}^2}}
\def\xb{{\tilde x}}
\def\ab{{\tilde a}}
\def\pb{{\tilde p}}
\def\bb{{\tilde \beta}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\half}{\frac{1}{2}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\edth}{{\p \!\!}'}
\newcommand{\koniec}{\begin{flushright}  $\Box $ \end{flushright}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\newcommand{\Section}[1]{\section{#1} \setcounter{equation}{0}}
\def\theequation{\thesection.\arabic{equation}}
\def\ot{\otimes}
\def\t{\tilde}
\def\lie{\mbox{Lie}}
\def\pst{\widetilde {\phi}}
  \def\ps{\phi}
\def\psm{\mid \ps \mid}
\def\psb{\ov{\ps}}
\def\xm{\mid \xi \mid}
\def\ve{\varepsilon}
\def\os{\Om _{\Sm}}
\def\xib{\overline{\xi}}
\def\xit{\tilde{\xi}}
\def\Sm{\Sigma}
\def\Smt{\widetilde {\Sm}}
\def\s{\sigma} 
\def\th{\theta}
\def\const{\mbox{const}}
\def\r{\rho}
\def\v{\bf v}
\def\u{\bf u}
\newcommand{\e}{\textbf{e}}
\def\vv{\varepsilon}
\def\Om{\Omega}
\def\Th{\Theta}
\def\G{\Gamma}
\def\O{\cal O}
\def\OO{\cal O}
\def\om{\omega}
\def\Do{\p _0}
\def\dd{\p _2}
\def\ds{\d_{\Sigma}}
\def\ov{\overline}
\def\g{\mathfrak{g}}
\def\wt{\overline{w}}
\def\zt{\overline{z}}
\def\xt{\tilde x}
\def\yt{\overline{y}}
\def\tW{\overline{\bf W}}
\def\tZ{\overline{\bf Z}}
\def\Wt{\widetilde W}
\def\Zt{\widetilde Z}
\def\tw{\tilde w}
\def\tz{\tilde z}
\def\lt{\tilde{\lambda}}
%\def\yt{\tilde y}
\def\p{\partial}
\def\pt{\tilde \p}
\def\do{\p _0}
\def\dd{\p _2}
\newcommand{\spp}{\mathbb{S}}
\def\ov{\overline}
\def\pa{\pi_{A'}d\pi^{A'}}
\def\Kt{\tilde{K}}
\def\K{\kappa}
\def\sm{\sigma}
\def\M{{\cal M}}
\newcommand{\hook}{{\setlength{\unitlength}{11pt}   % adjust pt size here
                   \begin{picture}(.833,.8)
                   \put(.15,.08){\line(1,0){.35}}
                   \put(.5,.08){\line(0,1){.5}}
                   \end{picture}}}
\def\a{\alpha}
\def\l{\lambda}
\def\Pt{{\cal PT}}
\def\O{{\cal O}}
\def\at{\tilde \a}
\def\dom{\delta \Om}
\def\tom{\tilde{\omega}}
%\def\ddot{\delta \Theta}
\def\macierz{
\left (
\begin{array}{cccc}
0&1&0&0\\
1&0&0&0\\
0&0&0&1\\
0&0&1&0
\end{array}
\right )
}
\def\pa{\pi_{A'}d\pi^{A'}}
\def\con{\,\rule{5.5pt}{0.3pt}\rule{0.3pt}{5.5pt}\,}
%\def\con1{\,\rule[5.5pt]{5.5pt}{0.3pt}\rule{0.3pt}{5.5pt}\,}
\def\Kt{\widetilde{K}}
\newtheorem{theo}{Theorem}[section] 
\newtheorem{prop}[theo]{Proposition}  
\newtheorem{lemma}[theo]{Lemma}
\newtheorem{defi}[theo]{Definition}
\newtheorem{col}[theo]{Corollary}
\newtheorem{ex}[theo]{Example}
\newtheorem{Conj}[theo]{Conjecture}
%\topmargin-0.5in
%\headheight0pt
%\headsep0pt
\oddsidemargin0pt
%\textheight21cm
\textwidth17cm
%\linespread{1.6}
